The Change-of-Measure Method, Block Lewis Weights, and Approximating Matrix Block Norms

Given a matrix $\mathbf{A} \in \mathbb{R}^{k \times n}$, a partitioning of $[k]$ into groups $S_1,\dots,S_m$, an outer norm $p$, and a collection of inner norms such that either $p \ge 1$ and $p_1,\dots,p_m \ge 2$ or $p_1=\dots=p_m=p \ge 1/\log n$, we prove that there is a sparse weight vector $\mathbf{\beta} \in \mathbb{R}^{m}$ such that $\sum_{i=1}^m \mathbf{\beta}_i \cdot \|\mathbf{A}_{S_i}\mathbf{x}\|_{p_i}^p \approx_{1\pm\varepsilon} \sum_{i=1}^m \|\mathbf{A}_{S_i}\mathbf{x}\|_{p_i}^p$, where the number of nonzero entries of $\mathbf{\beta}$ is at most $O_{p,p_i}(\varepsilon^{-2}n^{\max(1,p/2)}(\log n)^2(\log(n/\varepsilon)))$. When $p_1\dots,p_m \ge 2$, this weight vector arises from an importance sampling procedure based on the \textit{block Lewis weights}, a recently proposed generalization of Lewis weights. Additionally, we prove that there exist efficient algorithms to find the sparse weight vector $\mathbf{\beta}$ in several important regimes of $p$ and $p_1,\dots,p_m$. Our results imply a $\widetilde{O}(\varepsilon^{-1}\sqrt{n})$-linear system solve iteration complexity for the problem of minimizing sums of Euclidean norms, improving over the previously known $\widetilde{O}(\sqrt{m}\log({1/\varepsilon}))$ iteration complexity when $m \gg n$. Our main technical contribution is a substantial generalization of the \textit{change-of-measure} method that Bourgain, Lindenstrauss, and Milman used to obtain the analogous result when every group has size $1$. Our generalization allows one to analyze change of measures beyond those implied by D. Lewis's original construction, including the measure implied by the block Lewis weights and natural approximations of this measure.

==> notes.tex <==
%%%% CUSTOM ANALYSIS OF IPM

\subsection{Log-barrier interior point method with multiplicative approximation}

Although the analysis entailed by \Cref{lemma:ipm_log_barrier} is standard and easily follows from the self-concordance framework developed by \citet{nesterov1994interior}, we could not find an analysis that yields a multiplicative approximation guarantee. Hence, we include it for completeness.

First, we transform \eqref{eq:msn} into a constrained
minimization problem:
\begin{align*}
    \min~& \sum_{i=1}^m \vc_i\\
    \text{s.t. } &\|\mA_{S_i} \vx - \vb_i\|_2 \le \vc_i \quad \text{for all } 1 \le i \le m&\\
    &\vx \in \R^n, ~ \vc \in \R^m_{\ge 0}
\end{align*}

Now, for the constraints we define the logarithmic barrier
$h(\vx, \vc) = -\sum_{i=1}^m \logv{\vc_i^2 - \norm{\mA_{S_i}\vx-\vb_i}_2^2}$.
Given \(t > 0\), our intermediate optimization problems on the central path are \(\min_{\vx, \vc} f_t(\vx, \vc)\), where we use \(f_t(\vx, \vc) \coloneqq t \cdot \sum_{i=1}^m \vc_i + h(\vx, \vc)\).

\begin{lemma}
\label{lemma:log_barrier_sc}
The barrier \(h(\vx,\vc)\) is $2m$-self-concordant.
\end{lemma}
\begin{proof}[Proof of \Cref{lemma:log_barrier_sc}]
If \(h_i(\vx, \vc_i) \coloneqq -\logv{\vc_i^2 - \norm{\mA_{S_i} \vx - \vb_i}_2^2}\) is self-concordant,
the Lemma follows as \(h\) is a sum of self-concordant functions.
This is a barrier for the second-order cone composed with an affine transformation.
This barrier for the second-order cone is $2$-self-concordant as shown in \cite[Proposition 5.4.3]{nesterov1994interior},
and pre-composing with an affine transformation does not change self-concordance \cite[Proposition 2.1.1]{nesterov1994interior}. Thus, $\sum h_i$ is $2m$ self-concordant, completing the proof of \Cref{lemma:log_barrier_sc}.
\end{proof}

Next, we derive a reduced objective that we can optimize that bakes in the optimal values of $\vc$ for a fixed $t$.

\begin{lemma}
\label{lemma:reduced_obj}
For $t > 0$, the minimizing $\vc$ for $f_t(\vx, \vc)$ is given by
\begin{align*}
    \vc_i = \frac{1}{t} + \sqrt{\frac{1}{t^2} + \norm{\mA_{S_i}\vx-\vb_i}_2^2},
\end{align*}
and therefore minimizing $f_t(\vx,\vc)$ for a fixed $t > 0$ is equivalent to minimizing
\begin{align*}
    f_t(\vx) \coloneqq \sum_{i=1}^m \sqrt{1+t^2\norm{\mA_{S_i}\vx-\vb_i}_2^2} - \sum_{i=1}^m \logv{1+ \sqrt{1+t^2\norm{\mA_{S_i}\vx-\vb_i}_2^2}}
\end{align*}
for the same $t$.
\end{lemma}
\begin{proof}[Proof of \Cref{lemma:reduced_obj}]
The derivation essentially follows \cite[Appendix D]{clmps16}. By convexity, the optimal $\vc_i$ must be such that their partial derivatives are $0$. Hence, we study $\nabla_{\vc_i} f_t(\vx,\vc)$ and set it to $0$. Applying the chain rule to execute the differentiation, we get the equation
\begin{align*}
    t - \frac{2\vc_i}{\vc_i^2 - \norm{\mA_{S_i}\vx-\vb_i}_2^2} = 0,
\end{align*}
so applying the quadratic formula and taking the positive root gives
\begin{align*}
    \vc_i = \frac{1}{t} + \sqrt{\frac{1}{t^2} + \norm{\mA_{S_i}\vx-\vb_i}_2^2}.
\end{align*}
To derive the reduced objective, we plug this back into $f_t(\vx,\vc)$ and remove terms that are constant in $\vx$. We get
\begin{align*}
    f_t(\vx,\vc) &= t \sum_{i=1}^m \vc_i - \sum_{i=1}^m \logv{\vc_i^2-\norm{\mA_{S_i}\vx-\vb_i}_2^2} \\
    &= \sum_{i=1}^m \inparen{1+\sqrt{1+t^2\norm{\mA_{S_i}\vx-\vb_i}_2^2}} - \sum_{i=1}^m \logv{\frac{2}{t^2}+\frac{2}{t}\sqrt{\frac{1}{t^2}+\norm{\mA_{S_i}\vx-\vb_i}_2^2}} \\
    &= t + \sum_{i=1}^m \sqrt{1+t^2\norm{\mA_{S_i}\vx-\vb_i}_2^2} - m\logv{\frac{2}{t^2}} - \sum_{i=1}^m \logv{1+\sqrt{1+t^2\norm{\mA_{S_i}\vx-\vb_i}_2^2}},
\end{align*}
which completes the proof of \Cref{lemma:reduced_obj}.
\end{proof}

Next, in order to show that each Newton step has a convenient form, we take the gradient and the Hessian of the reduced objective $f_t(\vx)$.

\begin{lemma}
\label{lemma:reduced_obj_derivatives}
We have
\begin{align*}
    \nabla f_t(\vx) &= \sum_{i=1}^m t^2\inparen{1 - \frac{1}{1+ \sqrt{1+t^2\norm{\mA_{S_i}\vx-\vb_i}_2^2}}}\frac{\mA_{S_i}^{\top}\inparen{\mA_{S_i}\vx-\vb_i}}{\sqrt{1+t^2\norm{\mA_{S_i}\vx-\vb_i}_2^2}}\\
    \nabla^2 f_t(\vx) &= \mA^{\top}\mD\mA,
\end{align*}
where $\mD$ is a block-diagonal matrix where each block has size $\abs{S_i} \times \abs{S_i}$.
\end{lemma}
\begin{proof}[Proof of \Cref{lemma:reduced_obj_derivatives}]
For simplicity, let $g_i(\vx) \coloneqq 1+ \sqrt{1+t^2\norm{\mA_{S_i}\vx-\vb_i}_2^2}$. Then, we have
\begin{align*}
    f_t(\vx) = -t + \sum_{i=1}^m (g_i(\vx) - \logv{g_i(\vx)}).
\end{align*}
Thus,
\begin{align*}
    \nabla f_t(\vx) = \sum_{i=1}^m \inparen{\nabla g_i(\vx) - \frac{\nabla g_i(\vx)}{g_i(\vx)}}
\end{align*}
and
\begin{align*}
    \nabla^2 f_t(\vx) &= \sum_{i=1}^m \inparen{\nabla g_i(\vx)\nabla g_i(\vx)^{\top} - \frac{g_i(\vx) \cdot \nabla^2 g_i(\vx) - \nabla g_i(\vx)\nabla g_i(\vx)^{\top}}{g_i(\vx)^2}} \\
    &= \sum_{i=1}^m \inparen{\nabla g_i(\vx)\nabla g_i(\vx)^{\top}\inparen{1+\frac{1}{g_i(\vx)^2}}-\frac{\nabla^2 g_i(\vx)}{g_i(\vx)}}.
\end{align*}
Now, notice that
\begin{align*}
    \nabla g_i(\vx) = t^2 \cdot \frac{\mA_{S_i}^{\top}\inparen{\mA_{S_i}\vx-\vb_i}}{\sqrt{1+t^2\norm{\mA_{S_i}\vx-\vb_i}_2^2}} = t^2 \cdot \frac{\mA_{S_i}^{\top}(\mA_{S_i}\vx-\vb_i)}{g_i(\vx)-1}
\end{align*}
and
\begin{align*}
    \nabla^2 g_i(\vx) = t^2 \cdot \frac{(g_i(\vx)-1) \cdot \mA_{S_i}^{\top}\mA_{S_i}-\mA_{S_i}^{\top}\inparen{\mA_{S_i}\vx-\vb_i}\nabla g_i(\vx)^{\top}}{\inparen{g_i(\vx)-1}^2}.
\end{align*}
We now prove that $\nabla^2 f_t(\vx)$ has the promised structure. Let $\vv_i \coloneqq \mA_{S_i}\vx-\vb_i \in \R^{\abs{S_i}}$. This means that
\begin{align*}
    \nabla g_i(\vx) &= t^2 \cdot \frac{\mA_{S_i}^{\top}\vv_i}{g_i(\vx)-1} \\
    \nabla^2 g_i(\vx) &= t^2 \cdot \inparen{\frac{\mA_{S_i}^{\top}\mA_{S_i}}{g_i(\vx)-1} - t^2 \cdot \frac{\mA_{S_i}^{\top}\vv_i\vv_i^{\top}\mA_{S_i}}{\inparen{g_i(\vx)-1}^3}} = \frac{t^2}{g_i(\vx)-1} \cdot \inparen{\mA_{S_i}^{\top}\inparen{\mI_{\abs{S_i}}-\frac{t^2\vv_i\vv_i^{\top}}{\inparen{g_i(\vx)-1}^2}}\mA_{S_i}},
\end{align*}
and each term in the sum forming $\nabla^2 f_t(\vx)$ has the form
\begin{align*}
    &\quad \nabla g_i(\vx)\nabla g_i(\vx)^{\top}\inparen{1+\frac{1}{g_i(\vx)^2}}-\frac{\nabla^2 g_i(\vx)}{g_i(\vx)}\\
    &= \inparen{1+\frac{1}{g_i(\vx)^2}}\inparen{\mA_{S_i}^{\top}\inparen{\frac{t^4\vv_i\vv_i^{\top}}{(g_i(\vx)-1)^2}}\mA_{S_i}} - \frac{t^2}{g_i(\vx)(g_i(\vx)-1)} \cdot \inparen{\mA_{S_i}^{\top}\inparen{\mI_{\abs{S_i}}-\frac{t^2\vv_i\vv_i^{\top}}{\inparen{g_i(\vx)-1}^2}}\mA_{S_i}} \\
    &= \mA_{S_i}^{\top}\mM_i\mA_{S_i},
\end{align*}
where $\mM_i \in \R^{\abs{S_i} \times \abs{S_i}}$. Adding everything up yields the statement of \Cref{lemma:reduced_obj_derivatives}. 
\end{proof}

\Cref{lemma:reduced_obj_derivatives} easily implies that each Newton step reduces to solving linear systems in matrices $\mA^{\top}\mD\mA$ for block-diagonal matrices $\mD$, where each block has size $\abs{S_i} \times \abs{S_i}$. We now give a bound on the total number of Newton iterations of the barrier method assuming an initial point near the central path and path parameter $(\vx_0,t_0)$.

\begin{lemma}
\nnote{Apply the convergence analysis from \cite[Section 11.5.3]{boyd2004convex} with the target duality gap as $\eps \cdot \mathsf{OPT}$. Total number of Newton steps, i.e., system solves (to show this, explicitly compute what a Newton step looks like by taking the Hessian of $f_t(\vx) \coloneqq \sum_{i=1}^m \vc_i + (1/t) \cdot B(\vx,\vc)$), is given by (11.27)}
\[\widetilde{O}\inparen{\sqrt{m} \log(\nfrac{1}{\eps \cdot OPT}) \log(GR/|p^*|) \log(M-p*)}\]
(still need to interpret these)
\end{lemma}
\begin{proof}
\[\nabla^2 h_i(\vx, c_i) = \begin{bmatrix} 1 \\ \mA_{S_i}\end{bmatrix}^\top \cdot \inparen{\frac{c_i^2 - \norm{\mA_{S_i} \vx - \vb_i}_2^2}{2} \begin{bmatrix}
-1 & 0 \\
0 & \mI_{|S_i|}
\end{bmatrix} + \begin{bmatrix}
c_i^2 & c_i \vb_i^\top \\
c_i \vb_i & \vb_i \vb_i^\top
\end{bmatrix}} \cdot \begin{bmatrix}
    1 \\
    \mA_{S_i}
\end{bmatrix}\]
\end{proof}

\begin{lemma}
\nnote{Choose $t_0$, see \cite[Page 570-571]{boyd2004convex}}
\end{lemma}

%%%% OLD TECHNICAL OVERVIEW

\subsection{Technical overview}
\label{sec:overview}

In this subsection, we give a bird's eye view of the technical methods behind our proof of \Cref{thm:one_shot_lewis}.

\subsubsection{Concentration}
\label{sec:overview_concentration}

We begin with an explanation of our concentration argument. This type of argument has become standard in the line of work on sparsification (particularly in \cite{lee22,jlls23}), but we include a description for completeness.

We want to control the worst-case relative error of our sampling scheme. Let $\cG'$ be the dataset we obtain after we randomly sample indices $i_1,\dots,i_{\mtilde}$ to construct $\cM$, and define $\norm{\cdot}_{\cG'}$ similarly to $\norm{\cdot}_{\cG}$. By a standard argument, it is enough to prove that our sampling scheme obtains an \textit{additive} approximation for every $\vx \in B_{p} \coloneqq \{\vx\in\R^n\suchthat\gnorm{\mA\vx}{p}\le 1\}$. Hence, our task amounts to understanding $\E\sup \left|\| \mA\vx\|_{\cG_p}^p - \|\vx\|_{\cG'}^p \right|$.

We can start with calculating the probability that for a \textit{fixed} $\vx \in \R^n$, we have $\abs{\gnorm{\mA\vx}{p}^p-\norm{\vx}_{\cG'}^p} \le \eps$. This follows in a straightforward way from Bernstein's inequality. We can then consider a discretization of $B_{p}$ of resolution roughly $\eta$ and take a union bound over this discretization to bound the failure probability on the whole set $B_{p}$.

However, this incurs an extra factor of $n$ in our sparsity, coming from the fact that the discretization will have size roughly $\eta^{-n}$. To avoid this, we build a sequence of finer and finer approximations to every point in $B_{p}$ and consider the worst case ``chain'' of approximations for any $\vx \in B_{p}$. For an explanation of this theory, see the book by \citet{tal21}.

With this in hand, we can try to control the behavior of $\E\sup \left|\| \mA\vx\|_{\cG_p}^p - \|\vx\|_{\cG'}^p \right|$ over some finite set $T$. If we know tail bounds on the random variable $\left|\| \mA\vx\|_{\cG_p}^p - \|\vx\|_{\cG'}^p \right|$, then we can convert this into a bound on the expected maximum of the random process on a finite set. An argument of this sort yields the well-known fact that the maximum of $N$ random variables with Gaussian-like tail decay $\expv{-v^2}$ (i.e., subgaussian random variables) is roughly $\sqrt{\log N}$. At this point, we hope that for a discretization of size $2^{2^N}$, we only incur a small additional loss arising from the approximation. Denote this approximation error arising from a discretization of size $2^{2^N}$ as $e_N$ (which are known as \textit{entropy numbers} -- see Definition \ref{defn:entropy_numbers}) and then observe that our total error from the chain is roughly $\sum_{N \ge 0} 2^{N/2}e_N$. Although we glossed over many details, this sketch loosely captures the intuition behind \textit{Dudley's integral} for bounding the suprema of subgaussian processes. % $\exv{\sup \abs{\gnorm{\mA\vx}{p}^p - \norm{\vx}_{\cG'}^p}}$

By a standard symmetrization argument, it follows that it suffices to fix $i_1,\dots,i_{\mtilde}$ and argue that for independent $R_1,\dots,R_{\mtilde}$ where $R_h \sim \mathsf{Unif}\inparen{\pm 1}$ we have
\begin{align}
    \exvv{R_h}{\sup_{\vx \in B_{p}} \abs{\sum_{h=1}^{\mtilde} R_h \cdot \frac{\norm{\mA_{S_{i_h}}\vx}_{p_{i_h}}^p}{\vrho_{i_h}}}} \le \mtilde\cdot\eps.\label{eq:intro_empirical_process}
\end{align}
Intuitively, this means that for some appropriate rebalancing of the groups (given by the $\vrho_{i_h}$), a Rademacher average of the groups evaluated on every point in $\vx$ is close to $0$. It is straightforward to check that the above instantiation is a subgaussian process with respect to the distance
\begin{align*}
    \dtwo(\vx,\xhat) \coloneqq \inparen{\sum_{h=1}^{\mtilde} \inparen{\frac{\norm{\mA_{S_{i_h}}\vx}_{p_{i_h}}^p}{\vrho_{i_h}} - \frac{\norm{\mA_{S_{i_h}}\xhat}_{p_{i_h}}^p}{\vrho_{i_h}}}^2}^{1/2}.
\end{align*}
Our task is to now compute the entropy numbers $e_N(B_{p},\dtwo)$. It is in this calculation that we leverage the covering number estimates we develop in \Cref{sec:coverings} (see Sections \ref{sec:overview_geometry} and \ref{sec:overview_measure} for a sketch of how we derive these estimates).

\subsubsection{Covering numbers}
\label{sec:overview_geometry}

Now, we see that the main technical challenge that will emerge from the concentration argument (\Cref{sec:generic_chaining}) involves carefully controlling certain covering numbers. We explain this further. We first define the sampling body (\Cref{defn:sampling_polyhedron}).

\begin{definition}[Sampling body]
\label{defn:sampling_polyhedron}
Let $S$ be some subset of $[m]$ and $\vrho_1,\dots,\vrho_m$ be a probability distribution. Define the norm $\polynorm{\vx} \coloneqq \max_{i \in S} \vrho_i^{-1/p}\norm{\mA_{S_i}\vx}_{p_i}$. We call the unit norm ball of $\polynorm{\vx}$ the \textit{sampling body}.
\end{definition}

Recall that the covering number $\cN(K_1,K_2)$ for two symmetric convex bodies $K_1$ and $K_2$ is the minimum number of translates of $K_2$ required to cover $K_1$. Additionally, recall from the previous subsection the notion of \textit{entropy numbers} (which we will define in \Cref{defn:entropy_numbers}). These answer the question, ``what is the smallest radius $\eta$ such that $\log\cN(K_1,\eta \cdot K_2) \le 2^N$ for fixed symmetric convex bodies $K_1,K_2$?'' We will reduce controlling \eqref{eq:intro_empirical_process} to bounding the entropy numbers
\begin{align*}
    e_N\inparen{\inbraces{\vx\in\R^n\suchthat\gnorm{\mA\vx}{p}\le 1}, \inbraces{\vx\in\R^n\suchthat\polynorm{\vx}\le 1}}
\end{align*}
when $N$ is rather small. This places us in the setting where a simple volume-based argument becomes suboptimal. In this range, the dual Sudakov inequality (\Cref{fact:sudakov}) is the technical workhorse that allows us to get sharper bounds than what we would get if we applied just a volume-based bound. It states that if $B$ is the Euclidean ball in $n$ dimensions and $K$ is some symmetric convex body in $n$ dimensions, then we have
\begin{align*}
    \log\cN(B,\eta K) \lesssim \eta^{-2} \exvv{\vg\sim\cN(0,\mI_n)}{\norm{\vg}_K}^2,
\end{align*}
where $\norm{\cdot}_K$ is the \textit{gauge norm} for $K$, defined by $\norm{\vx}_K \coloneqq \inf\inbraces{t > 0 \suchthat \vx/t \in K}$.

However, applying the dual Sudakov inequality requires that we analyze covering numbers of the form $\log\cN(B, K)$ where $B$ is the Euclidean ball in $n$ dimensions and $K$ is some symmetric convex body. Denoting $\{\vx\in\R^n\suchthat\polynorm{\vx}\le 1\}$ by $K$, we see that we cannot immediately apply the dual Sudakov inequality to bound $\log\cN(B_p,\eta K)$. This is because $B_p$ is not a (linear transformation of a) Euclidean ball. \citet{jlls23} resolve this by generalizing the dual Sudakov inequality to cover arbitrary symmetric convex bodies. Unfortunately, this approach is not optimal in every setting. One source of the loss arises from exploiting the concentration of Lipschitz functionals of isotropic log-concave random vectors -- improving the bounds on this concentration depends on further progress on the KLS conjecture. Another is that the one-dimensional marginals of isotropic log-concave random variables, without any further assumptions, are only subexponential.

To escape these inefficiencies, we will want to try to find a way to apply the dual Sudakov inequality as-is. We will then only have to resort to concentration of Lipschitz functionals of Gaussian random vectors, which we do have a tight understanding of (arising from the Gaussian isoperimetric inequality). A natural attempt is to first observe that for any $t > 0$,
\begin{align}
    \log\cN\inparen{B_p, \eta K} \le \log\cN\inparen{B_p, t\widehat{B_2}} + \log\cN\inparen{t\widehat{B_2}, \eta K} = \log\cN\inparen{B_p, t\widehat{B_2}} + \log\cN\inparen{\widehat{B_2}, \frac{\eta}{t}\cdot K}.\label{eq:intro_split_covering}
\end{align}
We will choose $\widehat{B_2}$ to be a linear transformation of a Euclidean ball so that we can control $\log\cN\inparen{\widehat{B_2}, \eta/t \cdot K}$ using the dual Sudakov inequality. 

Here, we will split our argument based on whether $p \ge 2$. When $p \ge 2$, it will become clear later on that it will be sufficient to choose $\widehat{B_2}$ so that $B_p \subseteq \widehat{B_2}$. Then, it is easy to see that when $t=1$, we get $\log\cN(B_p,t\widehat{B_2}) = 0$. Hence, we have $\log\cN(B_p, \eta K) \le \log\cN(\widehat{B_2}, \eta K)$, and the required bound will follow from exploiting the concentration of Lipschitz functionals of Gaussian random vectors and then applying the dual Sudakov inequality.

However, when $p < 2$, we are still left with a pesky $\log\cN(B_p,t \widehat{B_2})$ term. Loosely, this is almost dual to the statement of the dual Sudakov inequality. Now, because it is known that covering number duality does hold when one of the bodies in question is the Euclidean ball, it may be tempting to simply write $\log\cN(B_p, t\widehat{B_2}) = \log\cN(\widehat{B_2},t B_q)$ where $B_q$ is the dual ball to $B_p$ after applying some linear transformation to map $\widehat{B_2}$ to $B$. The challenge here is that we do not believe that the gauge of the resulting $B_q$ has a form that is amenable to analysis. We will therefore need to be more careful, and we describe our alternative approach in \Cref{sec:overview_measure}.

\subsubsection{The change-of-measure principle and norm interpolation}
\label{sec:overview_measure}

Recall from the previous part that our goal is to bound $\log\cN(B_p,t\widehat{B_2})$ when $p < 2$.

We are now ready to introduce our main conceptual message -- \textit{by changing the measure under which we take norms, we can almost automatically identify a linear transformation of a Euclidean ball $\widehat{B_2}$ that is a good approximation to $B_p$}. We remark that this sort of idea has already been used by \citet{blm89} and \citet{sz01} to obtain the required $\widehat{B_2}$ in the special case where all the $S_i$ are singletons. Our goal is to generalize this machinery to give similar results for the block norm sampling problem.

Let us describe this idea further. Let $\vlambda_1,\dots,\vlambda_m$ denote a probability measure over the groups. Let $\mLambda \in \R^{k\times k}$ be the diagonal matrix such that if $j \in S_i$, then $\mLambda_{jj} = \vlambda_i$. Finally, for any $r > 0$ and $\vy\in\R^k$, let $\gnorml{\vy}{r} = (\sum_{i \le m} \vlambda_i\norm{\vy}_{p_i}^{r})^{1/r}$ and $B_r \coloneqq \{\vx\in\R^n \suchthat \gnorml{\mLambda^{-1/p}\mA\vx}{r} \le 1\}$. Notice that under this definition, we  still have \(B_p\) as before. We will first describe the argument when the groups are singletons, then explain how to move onto the general case. We will take $\widehat{B_2} = B_2$; it is easy to see that this is a linear transformation of a Euclidean ball.

Next, notice that by log-convexity of norms, if we choose $0 < \theta < p$ and $r > 2$ for which $1/2 = (\theta/2)/p + (1-\theta/2)/r$, we have
\begin{align}
    \gnorml{\vy}{2}^2 \le \gnorml{\vy}{p}^{\theta} \cdot \gnorml{\vy}{r}^{2-\theta}.\label{intro:compact_rounding_interpolation}
\end{align}
We will exploit this observation as follows. We will show that there exists a set $\cL_k$ that is (a subset of) the unit ball of $B_2$ such that every pair of points in $\cL_k$ is $\delta_k$-separated according to $\gnorml{\cdot}{r}$, where we will find $\delta_k$ according to the interpolation inequality \eqref{intro:compact_rounding_interpolation}. Furthermore, we will generate $\cL_k$ using a sort of compactness argument arising from a $B_2$-maximally separated subset of $B_p$. This means we get, for every $k \ge 0$,
\begin{align*}
    \log\cN(\widehat{B_2}, \delta_k B_r) \ge \log\abs{\cL_k} \ge \logv{\frac{\cN(B_p,8^k t \widehat{B_2})}{\cN(B_p, 8^{k+1} t \widehat{B_2})}},
\end{align*}
and then summing over $k \ge 0$ (noting that once $k$ is sufficiently large, $\cN(B_p, 8^kt \widehat{B_2}) = 1$), we have
\begin{align*}
    \log\cN(B_p, t\widehat{B_2}) \le \sum_{k \ge 0} \log\cN(\widehat{B_2},\delta_k B_r).
\end{align*}
Notice that the right hand side can be evaluated using the dual Sudakov inequality\footnote{For technical reasons that will be clearer in \Cref{sec:coverings}, we will have to do this after another interpolation step.} (recall the previous section), so it suffices to show that $\log\cN(\widehat{B_2},\eta B_r)$ is small.

This is where the choice of measure becomes crucial. Since both $\widehat{B_2}$ and $B_r$ are dependent on our choice of measure $\vlambda$, we will need to carefully choose the measure so that our covering numbers are well-behaved. A classical result of \citet{Lewis1978} establishes the existence of a change-of-measure under which we simultaneously get, for all $r \ge 2$,
\begin{align*}
    B_r \subset \widehat{B_2} \subset n^{1/2-1/r}B_r.
\end{align*}
Readers familiar with the work of \citet{cp15} may observe that this change-of-measure corresponds to the ``$\ell_p$ Lewis weights'' of $\mA$ (in particular, if $\vw_i$ is the $i$th $\ell_p$ Lewis weight, then we get $\vlambda_i = \vw_i/n$). It will turn out that this choice of $\vlambda$ is enough for us to ensure that $\cN(\widehat{B_2}, \eta B_r)$ is sufficiently small for our purposes.

\paragraph{Handling general $S_i$.} The main challenge with directly porting this argument to the block norm sampling problem is that $B_2$ is not a linear transformation of a Euclidean ball. We will therefore have to choose $\widehat{B_2}$ to be a ``rounding'' of $B_2$ such that $B_2 \subseteq \widehat{B_2}$. Observe that the interpolation step \eqref{intro:compact_rounding_interpolation} will continue to hold here, as we will get $\norm{\vy}_{\widehat{B_2}} \le \gnorml{\vy}{2}$. However, if $\widehat{B_2}$ is chosen suboptimally, then there could a large loss in the interpolation step \eqref{intro:compact_rounding_interpolation}.

Fortunately for us, through the proof of Lemma 4.2 of \cite{jlls23}, we will be able to extract a measure $\vlambda$ and a $\widehat{B_2}$ such that we get $B_2 \subseteq \widehat{B_2}$. Moreover, these objects arise from the stationary conditions of an optimization program that is the natural generalization of the one studied in \cite{sz01} to extend Lewis's measure construction to the range $0 < p < 1$ (for this reason, the authors call their importances the \textit{block Lewis weights}). After applying this change-of-measure, the control we get over $\log\cN(\widehat{B_2},\eta B_r)$ is essentially as good as what we get in the case where all the $S_i$ are singletons. In this sense, perhaps surprisingly, the group norm sampling problem does not have significantly worse bounds than the vanilla row sampling problem.

It remains to actually execute this change-of-measure procedure. The arguments of \citet{blm89} and \citet{sz01} appear to use specific properties of Lewis's change of measure. However, upon closer inspection, this is not really the case. This sort of argument can be generalized so that we get a general covering number formula under \textit{any} choice of probability measure, even when $0 < p < 1$. The results we need will follow from plugging in the measure implied by Lemma 4.2 of \cite{jlls23} into our formula. Finally, estimating $\norm{\vg}_{B_r}$ for $\vg \sim \cN(0,\mI_n)$ is a matter of applying again the fact that the concentration of Lipschitz functionals of Gaussian vectors is determined entirely by the Lipschitz parameter of the functional.


\paragraph{Change-of-measures in functional analysis.} We end this section by noting that other change-of-measure arguments are used throughout the study of finite-dimensional subspaces of $L_p$, as they are a very useful way to compare the $L_p$ norm to some other norm of interest. See Section 1.2 of the survey by \citet{js01} for more information.
